Learning Discourse-level Diversity for Neural Dialog Models using Conditional Variational Autoencoders

While recent neural encoder-decoder models have shown great promise in modeling open-domain conversations, they often generate dull and generic responses. Unlike past work that has focused on diversifying the output of the decoder at word-level to alleviate this problem, we present a novel framework based on conditional variational autoencoders that captures the discourse-level diversity in the encoder. Our model uses latent variables to learn a distribution over potential conversational intents and generates diverse responses using only greedy decoders. We have further developed a novel variant that is integrated with linguistic prior knowledge for better performance. Finally, the training procedure is improved by introducing a bag-of-word loss. Our proposed models have been validated to generate significantly more diverse responses than baseline approaches and exhibit competence in discourse-level decision-making.

==> backup.tex <==
However, first of all, from practical reasons, direct decoding from their objective function $(1-\lambda)\log p(T|S)+\lambda \log p(S|T)$ is intractable due to the enormous search space for target response. Meanwhile, the model results in non-globally-optimal solution since it fully depends on system's success in generating a sufficiently diverse N-best list. Secondly, their models have been focused on the algorithmic dimensions of the problem and are unable to explicitly model holistic properties of the sentence such topic, sentiment or topic. Our work addressed these problems through introducing latent factors of a conversation in the proposed kgCVAE models, which could extensively capture different properties of dialogues. 

Beam search optimization is widely used to generate diversified outputs for neural conversational model~\cite{serban2016building}. Wiseman and Rush~\shortcite{wiseman2016sequence} attempted to solve two major biases of seq2seq models that lead to monotonous output: exposure bias and loss-evaluation mismatch.  To remedy these, first of all, their modified seq2seq models produce scores for ranking sentences rather than predicting the probabilities of next word. Then they introduced search-based loss for RNN training and keep full gold sequence to be at the top of the beam through recording margin violation in forward pass and backpropagating errors in backward pass. This beam search algorithm is slow and has not been proved to be able to scale up.

Pavel et al,.~\shortcite{sountsov2016length} proposed an alternative model to achieve globally conditioning the $p(y|x)$ distribution. They argued that seq2seq models exhibit a bias towards short sequences that surprisingly gets worse with increasing beam size. This counter-intuitive phenomena is due to a margin discrepancy in the training loss of encoder-decoder models. Their model includes two RNN encoders to project both inputs and outputs into fixed-length vectors, which produces better calibrated sequence-level probabilities and alleviate bias issues of outputs. However, their model requires a closed space of allowed outputs and their proposed architecture is not able to generate responses directly. 

\cite{li2016persona} intend to add more contexts in neural response generation by presenting persona-based models to address speaker consistency . They captured individual characteristics by encoding background information and speaking style into the distributed embeddings, which is used to rerank the generated response from sequence-to-sequence model.

\cite{li2016deep} pointed out maximum-likelihood estimation(MLE) objective function of sequence-to-sequence model is unable to approximate the real-world goal of conversation. Thus, they initilized sequence-to-sequence model with MLE estimation and leveraged reinforcement learning to optimize three useful conversational properties such as informativity, coherence, and ease of answering. 


Moreover, in order to confirm that our training objective indeed strives to capture such discourse information, we collect the posterior $z$ for every utterance in the test dataset at each stage of the training and deploy a linear classifier as a probe~\cite{zhao2016towards} the amount of captured discourse information. Specifically, we use the posterior $z$ of $x$ as the inputs to a logistic regress or that is trained to predicts the dialog act and sentiment of $x$. 
\begin{table}[!htb]
    \centering
    \begin{tabular}{p{0.1\textwidth}|p{0.09\textwidth}p{0.09\textwidth}p{0.09\textwidth}} \hline 
    Models &  5K & 10K & 50K \\ \hline
    DA-Acc &  xx &  xx & xx \\ 
    Sent-Acc & xx & xx & xx\\ \hline
    \end{tabular}
    \caption{Performance of each model on automatic measures. }
    \label{tbl:latent}
\end{table}
Table~\ref{tbl:latent} shows the results. We can see after a model is better trained, the posterior $z$ indeed begins to capture more information that is beneficial for predicting the dialog act and sentiment of the predicting response $x$. 

\textbf{Connection to Conventional Dialog System Pipeline}: Our models are connected to the conventional dialog system pipeline~\cite{bohus2007olympus}. The context encoding network corresponds the natural language understanding and dialog state tracker, which produces a summarized representation of the dialog state. The prior network corresponds to the dialog manager that outputs a high-level action of the next response based on the dialog state. Then the decoder network plays the role of a context-sensitive natural language generator that produces the surface form of the prior network's outputs. Lastly the recognition network can be understood as a data-driven designer of the dialog systems, which discover useful high-level factors form the data and encode them in the latent variable $z$. This implies a promising research direction for data-driven dialog system (see Section~\ref{sec:implication} for details).


\subsection*{Consistence of Natural Language Generation}
Since kgCVAE first predicts the dialog act of the response, and then generate the response conditioned on both the context and its predicted dialog act, a natural evaluation is to measure the performance of kgCVAE in generating sentences that is consistent with its own dialog act prediction. We denote the predicted dialog act as $y\prime$ as the ground truth and the tagged dialog act based on the generated words from dialog act tagger as prediction. The accuracy on the test dataset is $80.5\%$, which suggest that kgCVAE is able to jointly model the relationship between the dialog act and its associated surface realization. 
\begin{table}[ht]
    \centering
    \begin{tabular}{p{0.35\textwidth}|p{0.05\textwidth}} \hline 
    Error Pair &  Error\\\hline
    s-non-opinion vs. s-opinion & 46.2\% \\
    uninterpretable vs. s-non-opinion & 8.7\% \\
    backchannel vs. agree/accept & 5.7\% \\
    backchannel vs. s-non-opinion & 5.2\%\\\hline
    \end{tabular}
    \caption{Most confusion pairs for kgCVAE generation. S is short handed for statement.}
    \label{tbl:diversity}
\end{table}


\subsection{Latent Space Analysis}
At last, we are interested in investigating the properties of the learned latent space $z$. We hypothesise that the posterior $z$ from the recognition network $q_\phi(z|x,y,c)$ captures important discourse information in the context response tuple ($c$, $x$). To verify this hypothesis, we first use t-SNE~\cite{maaten2008visualizing} to map the collected $z$ into 2-dimensional space and explored the potential clustering existed in the latent space. Figure~\ref{fig:tsne} shows our finding and they suggest that the latent space is correlated with the length, the sentiment and the dialog act of the encoding $x$.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.23\textwidth]{figures/da.png}
    \includegraphics[width=0.23\textwidth]{figures/senti.png}
    \caption{(Left) t-SNE of posterior $z$ against the dialog act. (Right) the color indicates the intensity of sentiment and the size of circle indicates the length of the encoding $x$. }
    \label{fig:tsne}
\end{figure}



==> implication.tex <==
\textbf{Connection to Conventional Dialog System Pipeline}: Our models are connected to the conventional dialog system pipeline~\cite{bohus2007olympus}. The context encoding network corresponds the natural language understanding and dialog state tracker, which produces a summarized representation of the dialog state. The prior network corresponds to the dialog manager that outputs a high-level action of the next response based on the dialog state. Then the decoder network plays the role of a context-sensitive natural language generator that produces the surface form of the prior network's outputs. Lastly the recognition network can be understood as a data-driven designer of the dialog systems, which discover useful high-level factors form the data and encode them in the latent variable $z$. This implies a promising research direction for data-driven dialog system (see Section~\ref{sec:implication} for details).
